Tiling by rectangles and alternating current

This paper is on tilings of polygons by rectangles. A celebrated physical interpretation of such tilings due to R.L. Brooks, C.A.B. Smith, A.H. Stone and W.T. Tutte uses direct-current circuits. The new approach of the paper is an application of alternating-current circuits. The following results are obtained: - a necessary condition for a rectangle to be tilable by rectangles of given shapes; - a criterion for a rectangle to be tilable by rectangles similar to it but not all homothetic to it; - a criterion for a generic polygon to be tilable by squares. These results generalize the ones of C. Freiling, R. Kenyon, M. Laczkovich, D. Rinne and G. Szekeres.

==> metal-fig6c.tex <==
\ctikzset{bipoles/length=.6cm}
\begin{circuitikz}[scale=0.3, american]
\draw[color=brown]
(-2.7,1) to[R, o-*] (0,4.66)
      to[R, *-*] (2.4,3.76)
      to[R, *-o] (6.9,1)
(-2.7,1) to[R, o-*] (1.5,-1.2)
      to[R, *-o] (6.9,1)
(-2.7,1) to[R, o-*] (0.3,1.8)
      to[R, *-*] (2.4,3.76)
(0,4.66) to[R, *-*]  (0.3,1.8)
      to[R, *-*] (1.5,-1.2)
%(6.9,1)  to[short, *-] (6.9,6.0)
%      to[battery, -] (-2.7,6.0)
%      to[short, -*] (-2.7,1)
;\end{circuitikz}

